TOI-836: A super-Earth and mini-Neptune transiting a nearby K-dwarf

We present the discovery of two exoplanets transiting TOI-836 (TIC 440887364) using data from TESS Sector 11 and Sector 38. TOI-836 is a bright ($T = 8.5$ mag), high proper motion ($\sim\,200$ mas yr$^{-1}$), low metallicity ([Fe/H]$\approx\,-0.28$) K-dwarf with a mass of $0.68\pm0.05$ M$_{\odot}$ and a radius of $0.67\pm0.01$ R$_{\odot}$. We obtain photometric follow-up observations with a variety of facilities, and we use these data-sets to determine that the inner planet, TOI-836 b, is a $1.70\pm0.07$ R$_{\oplus}$ super-Earth in a 3.82 day orbit, placing it directly within the so-called 'radius valley'. The outer planet, TOI-836 c, is a $2.59\pm0.09$ R$_{\oplus}$ mini-Neptune in an 8.60 day orbit. Radial velocity measurements reveal that TOI-836 b has a mass of $4.5\pm0.9$ M$_{\oplus}$ , while TOI-836 c has a mass of $9.6\pm2.6$ M$_{\oplus}$. Photometric observations show Transit Timing Variations (TTVs) on the order of 20 minutes for TOI-836 c, although there are no detectable TTVs for TOI-836 b. The TTVs of planet TOI-836 c may be caused by an undetected exterior planet.

==> 3.Results/results.tex <==
% \subsection{Densities} \label{sec:densities}

% As a result of our joint fitting of transit and radial velocity data, we find that \Tplanetb\ is a super-Earth planet with a radius of \TRadiusbshort\,\rearth\ and mass of \TMassbshort\,\mearth, on a period of \Tperiodbshort\,days, and \Tplanetc\ is a sub-Neptune planet with a radius of \TRadiuscshort\,\rearth\ and mass of \TMasscshort\,\mearth\, on a period of \Tperiodcshort\,days. From this we can infer a bulk density of \Tdensitybshort\,\gccc\ for \Tplanetb, and \Tdensitycshort\,\gccc\ for \Tplanetc. A full set of parameters for \Tstar\ can be found in Table \ref{tab:star_props_results}, and parameters for each planet can be found in Table \ref{tab:planet_props}.

% \begin{center}
% \begin{table}
%     \centering
%     \caption{Stellar parameters of \TStar.}
%     \label{tab:star_props_results}
%     \begin{threeparttable}
%     \begin{tabularx}{0.96\columnwidth}{ l  l X }
%     \toprule
%     \textbf{Property (unit)} & \textbf{Value} & \textbf{Source} \\
%     \hline
%     % \textbf{Key parameters} & & \\
%     Mass (\Msun)    & \Tstarmassexo & \texttt{exoplanet} \\
%     Radius (\Rsun)  & \Tstarradiusexo   & \texttt{exoplanet} \\
%     Density (\gccc) & \Tstardensityexo  & \texttt{exoplanet} \\
%     P\textsubscript{\textit{rot}} (days)   & \Tstarperiodexo   & \texttt{exoplanet} \\
%     \logg\ &\Tloggporto  &\texttt{ARES + MOOG + \gaia} \\
%     \teff\ (K)   &\Teffporto  &\texttt{ARES + MOOG} \\
%     \vsini\ (\kms) &\Tstarvsiniporto &\texttt{ARES + MOOG}\\
%     Age (Gyr)   &\Tstarageporto &Isochrones \\
%     % V\textsubscript{\textit{tur}} (\kms)    & \Tstarvturbporto  &Porto \\
% % \hline
% %     \textbf{Chemical abundance} &\textbf{Value (dex)} &\textbf{Source} \\
%     \hline
%     \multicolumn{3}{l}{\textbf{Stellar abundances}} \\
%     \feh\,(dex) &\Tstarfehporto &\texttt{ARES + MOOG} \\
%     \mgh\,(dex)   &\Tstarmghporto &\texttt{ARES + MOOG} \\
%     \sih\,(dex)    &\Tstarsihporto &\texttt{ARES + MOOG} \\
%     \hline
%     \multicolumn{3}{l}{\textbf{Galactic space velocity components}} \\
%     $U$ (\kms)   & -35.6 $\pm$ 0.7 & \gaia\ EDR3  \\
%     $V$ (\kms)  & -10.7 $\pm$ 0.3 & \gaia\ EDR3 \\
%     $W$ (\kms)  & -3.50 $\pm$ 0.5 & \gaia\ EDR3 \\
%     \bottomrule
%     \end{tabularx}
%     \begin{tablenotes}
%     \item Sources: \texttt{exoplanet} \citep{exoplanetdanforeman, exoplanetnew}, \texttt{ARES} \citep{sousa2015}, \texttt{MOOG} \citep{Sneden:1973, Kurucz:1993}
%     \end{tablenotes}
%     \end{threeparttable}
% \end{table}
% \end{center}


% \begin{center}
% \begin{table}
%     \centering
%     \caption{\hl{Parameters of} \Tplanetb\, \hl{and} \Tplanetc.}
%     \label{tab:planet_props}
%     \begin{tabular}{lll}
%     \toprule
%     \textbf{Property} & \multicolumn{2}{c}{\textbf{Value}} \\ \hline
%      & \multicolumn{1}{l}{\textbf{\Tplanetb}} & \multicolumn{1}{l}{\textbf{\Tplanetc}} \\
%     Identifier & TOI-836.02 & TOI-836.01 \\
%     Period (days) & \Tperiodb & \Tperiodc \\
%     Mass (\mearth) & \TMassb & \TMassc \\
%     Radius (\rearth) & \TRadiusb & \TRadiusc \\
%     Density (gccc) & \Tdensityb & \Tdensityc \\
%     R\textsubscript{\textit{p}}/R\textsubscript{*} & \Trorb & \Trorc \\
%     \tc\ (TBJD) & \Tcb & \Tcc \\
%     T1-T4 duration (hours) & \TTDurfullb & \TTDurfullc \\
%     T2-T3 duration (hours) & \TTDurcutb & \TTDurcutc \\
%     Impact parameter & \Timpactb & \Timpactc \\
%     \textit{K} (\ms) & \Tkb & \Tkc \\
%     Inclination ($^{\circ}$) & \Tincb & \Tincc \\
%     Semi-major axis (AU) & \Taub & \Tauc \\
%     Temperature T\textsubscript{\textit{eq}} (K) * & \Teqb & \Teqc \\
%     Insolation flux (\fsun) & \Tfluxb & \Tfluxc \\
%     Eccentricity & \Teccb & \Teccc \\
%     Argument of periastron ($^{\circ}$) & \Tomegab & \Tomegac \\
%     TSM & \TSMb & \TSMc \\
%     \bottomrule
%     \end{tabular}
% \end{table}
% \end{center}


% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{3.Results/Figures/CHEOPS_stacked_lightcurve_TOI-836.pdf}
%     \caption{\hl{Light curves of} \Tplanetb\ and \Tplanetc\ taken by the \cheops\ satellite as detailed in Table~\ref{tab:photobs}, plotted with our best fit \texttt{exoplanet} models for \Tplanetb\ in orange and \Tplanetc\ in blue, and offset for clarity.}
%     \label{fig:cheopslcs}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{3.Results/Figures/LCO_stacked_lightcurves_TOI-836.pdf}
%     \caption{\hl{Light curves of} \Tplanetb\ and \Tplanetc\ taken by the \lcogt\ network as detailed in Table~\ref{tab:photobs}, plotted with our best fit \texttt{exoplanet} models for \Tplanetb\ in orange and \Tplanetc\ in blue, and offset for clarity.}
%     \label{fig:lcolcs}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{3.Results/Figures/followup_stacked_lightcurve_TOI-836.pdf}
%     \caption{Lightcurves of \Tplanetc\ taken by the \MEarthSouth, \ngts\ and \astep\ facilities as detailed in Table~\ref{tab:photobs}, plotted with our best fit \texttt{exoplanet} models and offset for clarity.}
%     \label{fig:followuplcs}
% \end{figure}



% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{3.Results/Figures/dace1.png}
%     \caption{Radial velocity data of \Tstar\ from the \hires\ instrument on the \keck\ telescope from 2009 April 6 to 2013 February 3, and fit with a linear trend represented by the solid grey line.}
%     \label{fig:hiresdace}
% \end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \subsection{Transit timing variations} \label{results:ttv}

% \hl{We plot the resulting offset for the central transit time} \tc\ \hl{for each of} \Tplanetb\ and \Tplanetc\ \hl{in Figure}~\ref{fig:ttv}. We note that there appear to be no  significant TTVs in the observed transits of \Tplanetb, however in \Tplanetc\ we detect an offset within the \tc\ values ranging from approximately 20 to 30 minutes. The presence of these TTVs is supported by observations from both the space-based \cheops\ satellite and multiple ground-based facilities. These TTV measurements alone are not enough to be able to put meaningful constraints on the mass of \Tplanetc, but with further TTV monitoring it may be possible.
% %\textcolor{green}{Ed Bryant - any more ideas?}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\textwidth]{3.Results/Figures/ttv.png}
%     \caption{\hl{\textbf{Top panel:}} Transit Timing Variations (TTVs) for each transit of  \Tplanetb\ from the following photometry sources: \tess\ in turquoise and \cheops\ in yellow. \hl{\textbf{Bottom panel:}} Transit Timing Variations (TTVs) for each transit of  \Tplanetc\ from the following photometry sources: \tess\ in turquoise, \cheops\ in yellow, \lcogt\ in purple, \MEarthSouth\ in blue and \ngts\ in green.}
%     \label{fig:ttv}
% \end{figure}


% \subsection{Galactic kinematics} \label{results:galactic}

% %\textcolor{green}{Tom Wilson - SEE EMAIL, TW: Done}
% Following the formulation of \citet{johnson1987}, and using the values of proper motion and parallax from \gaia\ EDR3 (see Table \ref{tab:star_props}) and a radial velocity from \gaia\ DR2 of \GaiaRV\,\kms\ \citep{GAIA_DR2}, we calculate the values and uncertainties for $U$, $V$ and $W$, the heliocentric velocity components of the Galactic space velocities, in the direction of the galactic centre, rotation, and pole respectively, in Table \ref{tab:star_props_results}. We should note that we do not subtract the Solar motion and compute the $U$, $V$ and $W$ values in the right-handed system. %\textcolor{red}{please fill in sources column, TW: Done}

% We also use the approach of \citet{reddy2006} in a Monte Carlo fashion with 100,000 samples to determine the probability that \Tstar\ is in a given kinematic Galactic family, using a weighted average of the results obtained using the velocity dispersion standards of \citet{bensby2003, bensby2014}, \citet{reddy2006}, and \citet{chen2021}. We find a Galactic thin disk membership probability for \Tstar\ of 98.9\%, thick disk membership probability of 1.1\%, and halo membership probability of 0\%. This agrees well with the Galactic eccentricity of \Tstar\ of 0.08, and the high Galactic Z-component of the angular momentum of $Z$ $\approx$\,1770\,kpc\,\kms that we compute using the {\tt galpy} package after a Galactic orbit determination using the  \gaia\ EDR3 position, proper motions, and parallax, and \gaia\ DR2 radial velocity integrating over 5\,Gyr, as well as the typical values for \mgh\ and \sih\ from stellar analysis (see Section~\ref{sec:stellaranalysis}).
